Liouville Rigidity for Real and Complex Degenerate Hessian Equations

We prove Liouville rigidity theorems for translation-invariant real and complex Hessian equations in the viscosity sense, where the PDE is encoded by an admissible set $\mathcal{A}$. The main structural notion is Liouville admissibility, a recursive geometric condition requiring each quotient set to be either boundary compatible or to fall into a terminal class. Our main theorem states that every bounded, globally $C^{0,\alpha}$ entire viscosity solution of \[ \mathrm{Hess}_{\mathbb F}u\in\partial\mathcal{A} \] is constant if and only if $\mathcal{A}$ is Liouville admissible; thus the Liouville-type property is characterized as a geometric property of the admissible set. A central class of examples arises from polarizations of univariate G{\aa}rding polynomials satisfying the monotone root sequence condition, producing mixed elementary-symmetric admissible sets and recovering the standard $k$-Hessian equations as monomial cases. The framework also allows anisotropic constructions, including linear pullbacks and intersections of admissible sets.

==> Draft5-NotesonCurrents.tex <==
{\color{blue}
\section{Notes on weak solution in current sense}
\begin{definition}\autocite{MR3636634}
Let $u$ be a subharmonic function on a domain $\Omega\subset\mathbb{C}^n.$ Then $u$ is called $m$-subharmonic ($m$-sh for short) if for any collection of $C^2$-smooth $m$-sh functions $v_1,\ldots,v_{m-1}$ the inequality

$$dd^cu\wedge dd^cv_1\wedge\cdots\wedge dd^cv_{m-1}\wedge\beta^{n-m}\geq0$$
holds in the weak sense of currents.
The set of all $m$-sh functions is denoted by $\mathcal{SH}_m(\Omega).$
\end{definition}
\begin{definition}\autocite{MR3636634}
 An $m$-subharmonic function $u$ on a domain $\Omega$ is called maximal if for every $m$-subharmonic function $v$ and any compact set $K \subset \Omega$ the inequality $u \geq v$ on $\Omega \setminus K$ implies $u \geq v$ on $K$.
\end{definition}


\begin{proposition}\autocite{MR2172278}
    \begin{enumerate}
\item If $u$ is $C^2$ smooth then it is $m$-subharmonic if and only if the form $dd^c u$ belongs pointwise to $\widetilde{\Gamma}_m$;
\item If $u,v\in \mathcal{P}_m$ then $u+v\in \mathcal{P}_m$;
\item If $u\in \mathcal{P}_m$ and $\gamma\colon\mathbb{R}\to\mathbb{R}$ is a convex, increasing function then $\gamma\circ u\in \mathcal{P}_m$;
\item If $u$ is $m$-subharmonic then the standard regularizations $u*\rho_\varepsilon$ are also $m$-subharmonic;
\item If $\{u_\ell\}\subset \mathcal{P}_m$ is locally uniformly bounded from above then $\bigl(\sup_\ell u_\ell\bigr)^*\in \mathcal{P}_m$, where $v^*$ denotes the upper regularization of $v$;
\item $\operatorname{PSH}=\mathcal{P}_n\subset\cdots\subset \mathcal{P}_1=\operatorname{SH}$.
\end{enumerate}
\end{proposition}
\begin{theorem}\autocite{MR2172278}
Let $u$ be a bounded $m$-subharmonic function on a domain $\Omega$. Then $u$ is maximal if and only if
$$(dd^c u)^m \wedge \beta^{n-m} = 0$$
as measures.
\end{theorem}
The theorem above implies in particular that $m$-maximality of locally bounded $m$-sh function is a local property. 

Let
\[
\Gamma_m=\{\lambda\in\mathbb R^n:
\sigma_1(\lambda)>0,\ldots,\sigma_m(\lambda)>0\}
\]
and
\[
\mathcal A_m
=
\{H\in\operatorname{Herm}(n):\lambda(H)\in\overline{\Gamma_m}\},
\qquad
\Sigma_m=\partial\mathcal A_m.
\]

We claim that a continuous bounded maximal \(m\)-subharmonic function
is a viscosity solution of
\[
\Hess_{\mathbb C}u\in\Sigma_m.
\]

First, \(m\)-subharmonicity gives the viscosity subsolution condition
\[
\Hess_{\mathbb C}u\in\mathcal A_m.
\]
Indeed, if \(u\) is continuous and \(m\)-subharmonic, then its standard
regularizations \(u*\rho_\varepsilon\) are smooth \(m\)-subharmonic
on compact subsets and converge locally uniformly to \(u\). For smooth
functions, \(m\)-subharmonicity is equivalent to
\[
\lambda(\Hess_{\mathbb C}u)\in\overline{\Gamma_m}.
\]
Thus, by stability of viscosity subsolutions under locally uniform
convergence, \(u\) is a viscosity subsolution of
\[
\Hess_{\mathbb C}u\in\mathcal A_m.
\]

It remains to check the viscosity supersolution condition. Let
\(\varphi\in C^2\) touch \(u\) from below at \(z_0\). Suppose, for
contradiction, that
\[
\lambda(\Hess_{\mathbb C}\varphi(z_0))\in\Gamma_m
=
\operatorname{int}\overline{\Gamma_m}.
\]
By openness of \(\Gamma_m\) and continuity of \(\Hess_{\mathbb C}\varphi\),
for sufficiently small \(\varepsilon>0\) and \(r>0\), the function
\[
w(z)=\varphi(z)-\varepsilon |z-z_0|^2+\frac{\varepsilon r^2}{2}
\]
is \(m\)-subharmonic in \(B_r(z_0)\). Since \(\varphi\le u\) near
\(z_0\) and \(\varphi(z_0)=u(z_0)\), after choosing \(r\) small we have
\[
w\le u-\frac{\varepsilon r^2}{2}
\quad\text{on }\partial B_r(z_0),
\]
while
\[
w(z_0)=u(z_0)+\frac{\varepsilon r^2}{2}>u(z_0).
\]
This contradicts the maximality of \(u|_{B_r(z_0)}\). Therefore no
lower test function can have complex Hessian in \(\operatorname{int}
\mathcal A_m\). This is exactly the viscosity supersolution condition
for the boundary equation
\[
\Hess_{\mathbb C}u\in\Sigma_m.
\]

Consequently, a continuous bounded maximal \(m\)-subharmonic function
is a viscosity solution of
\[
\Hess_{\mathbb C}u\in\partial\mathcal A_m.
\]
In particular, the bounded Lipschitz maximal \(m\)-subharmonic functions
considered in \cite{MR3636634} are bounded uniformly Hölder viscosity
solutions of this boundary equation.

\bigskip

\bigskip

\bigskip

\bigskip

\bigskip

\bigskip


Next we quote from \cite{MR3600038} the following:
\begin{quote}
    ``In this paper we are interested in the case of $(n-1)$-plurisubharmonic functions (for $n\geqslant2)$, ($n-1)$-PSH for short, which can be characterized as follows. A $C^2$ function $u$ is $(n-1)$-PSH if the matrix whose $(i,j)$th entry is

$$\left(\sum_{k=1}^n\frac{\partial^2u}{\partial z^k\partial\overline{z}^k}\right)\delta_{ij}-\frac{\partial^2u}{\partial z^i\partial\overline{z}^j}$$

is non-negative definite.''

\dots \dots

   ``Let us say that a continuous $(n-1)$-PSH function $u$ is maximal if given any relatively compact open set $\Omega' \Subset \Omega$ and any continuous $(n-1)$-PSH function $v$ on a domain $\Omega''$ with $\Omega' \Subset \Omega'' \Subset \Omega$ and with $v \leq u$ on $\partial \Omega'$, and then we must have that $v \leq u$ on $\Omega'$.''

``Note that if $u$ is a continuous $(n-1)$-PSH and $\chi_\varepsilon$ is a family of mollifiers, we can define $u_\varepsilon = u * \chi_\varepsilon$. These are functions in $C^\infty(\Omega_\varepsilon)$, where $\Omega_\varepsilon = \{x \in \Omega \mid d(x, \partial \Omega) > \varepsilon\}$, which are also $(n-1)$-PSH since $P(u_\varepsilon) = P(u) * \chi_\varepsilon \geq 0$, and $u_\varepsilon \to u$ is locally uniform as $\varepsilon \to 0$.''
\end{quote}
\begin{theorem}\cite{MR3600038}
If $u\colon \mathbb{C}^n\to\mathbb{R}$ is an $(n-1)$-$\operatorname{PSH}$ function on $\mathbb{C}^n$ which is Lipschitz continuous, maximal, and satisfies
\[
\sup_{\mathbb{C}^n}\bigl(|u|+|\nabla u|\bigr)<\infty,
\]
then $u$ is constant.
\end{theorem}

In this case the relevant subequation is
\[
\mathcal A_{n-1}
=
\{H\in\operatorname{Herm}(n):P(H)\geq0\},
\qquad
P(H):=(\operatorname{tr}H)I-H.
\]
Thus the boundary equation is
\[
P(\Hess_{\mathbb C}u)\in\partial\operatorname{Herm}_+(n),
\]
or equivalently,
\[
P(\Hess_{\mathbb C}u)\geq0,
\qquad
\det P(\Hess_{\mathbb C}u)=0.
\]

The same argument shows that a continuous maximal \((n-1)\)-PSH
function in the sense of \cite{MR3600038} is a viscosity solution of
this boundary equation. Indeed, the subsolution condition follows from
the mollification property quoted above. For the supersolution
condition, let \(\varphi\in C^2\) touch \(u\) from below at \(z_0\).
If
\[
P(\Hess_{\mathbb C}\varphi(z_0))>0,
\]
then, for sufficiently small \(\varepsilon>0\) and \(r>0\),
\[
w(z)=\varphi(z)-\varepsilon |z-z_0|^2+\frac{\varepsilon r^2}{2}
\]
is still \((n-1)\)-PSH in \(B_r(z_0)\), because
\[
P(\Hess_{\mathbb C}w)
=
P(\Hess_{\mathbb C}\varphi)-(n-1)\varepsilon I
\]
remains positive definite. As before, \(w\le u\) on
\(\partial B_r(z_0)\) but \(w(z_0)>u(z_0)\), contradicting maximality.
Hence no lower test function can satisfy
\(P(\Hess_{\mathbb C}\varphi)>0\), which is precisely the viscosity
supersolution condition.

Therefore the weak solutions appearing in the Liouville theorem of
\cite{MR3600038} are viscosity solutions of the corresponding boundary
equation. In particular, their theorem applies to bounded Lipschitz
viscosity solutions of
\[
P(\Hess_{\mathbb C}u)\in\partial\operatorname{Herm}_+(n).
\]
}
